Rewriting the Self: User Perceptions of AI-Mediated Cognitive Reframing

Individuals are increasingly using AI for psychological support. One specific paradigm, AI-mediated cognitive reframing (AIM-CR), uses AI to automatically reframe users' negative thoughts ("I failed...") into more adaptive perspectives ("I am learning..."). While prior work suggests that AIM-CR tools reduce users' negative emotions, the complexities of AI automatically modifying users' personal narratives remain underexplored. In this work, we investigated these complexities through a mixed-methods study in which 28 participants engaged with an AIM-CR tool that reframed narratives about their stressors. Our findings suggest that participants had mixed perceptions of AIM-CR: although reframing reduced negative emotions for most participants, participants felt less ownership of, and less authenticity in, the reframed narratives. Participants perceived AIM-CR as a validating "mirror," as "another self" that could motivate or alienate them, or as an external social actor. These perceptions shaped therapeutic dynamics. We conclude by discussing design implications for future AIM-CR tools to better preserve user agency in narrative co-construction and more effectively support mental health and well-being.

==> sections/resources/demographics.tex <==
\begin{table}[h]
\centering
  \caption{Participant Demographics}
\begin{tabular}{|p{0.15\linewidth}|p{0.15\linewidth}|p{0.4\linewidth}|p{0.3\linewidth}|}
\hline
\textbf{Participant ID} & \textbf{Age Group} & \textbf{Ethnicity}& \textbf{Gender}\\
\hline

P1 & 18-25 & East Asian & Female \\ \hline
P2 & 26-34 & East Asian & Male \\\hline
P3 & 18-25 & East Asian & Female \\\hline
P4 & 26-34 & East Asian & Male \\\hline
P5 & 18-25 & South Asian & Female \\\hline
P6 & 18-25 & South Asian & Female \\\hline
P7 & 18-25 & Middle Eastern or North African (MENA) & Non-binary \\\hline
P8 & 26-34 & White & Male \\\hline
P9 & 26-34 & East Asian & Female \\\hline
P10 & 35-44 & White & Female \\\hline
P11 & 18-25 & South Asian & Non-binary \\\hline
P12 & 26-34 & Black or African American & Female \\\hline
P13 & 26-34 & East Asian & Male \\\hline
P14 & 18-25 & Southeast Asian & Female \\\hline
P15 & 18-25 & East Asian & Female \\\hline
P16 & 18-25 & East Asian & Male \\\hline
P17 & 26-34 & East Asian & Male \\\hline
P18 & 26-34 & East Asian & Male \\\hline
P19 & 26-34 & East Asian & Female \\\hline
P20 & 18-25 & East Asian & Female \\\hline
P21 & 26-34 & Southeast Asian & Male \\\hline
P22 & 18-25 & East Asian & Female \\\hline
P23 & 18-25 & South Asian & Male \\\hline
P24 & 26-34 & South Asian & Male \\\hline
P25 & 26-34 & White & Female \\\hline
P26 & 26-34 & Southeast Asian & Male \\\hline
P27 & 26-34 & White & Male \\\hline
P28 & 26-34 & Southeast Asian & Male \\

\hline


\end{tabular}


\end{table}
